DeepN-JPEG: A Deep Neural Network Favorable JPEG-based Image Compression Framework

As one of most fascinating machine learning techniques, deep neural network (DNN) has demonstrated excellent performance in various intelligent tasks such as image classification. DNN achieves such performance, to a large extent, by performing expensive training over huge volumes of training data. To reduce the data storage and transfer overhead in smart resource-limited Internet-of-Thing (IoT) systems, effective data compression is a "must-have" feature before transferring real-time produced dataset for training or classification. While there have been many well-known image compression approaches (such as JPEG), we for the first time find that a human-visual based image compression approach such as JPEG compression is not an optimized solution for DNN systems, especially with high compression ratios. To this end, we develop an image compression framework tailored for DNN applications, named "DeepN-JPEG", to embrace the nature of deep cascaded information process mechanism of DNN architecture. Extensive experiments, based on "ImageNet" dataset with various state-of-the-art DNNs, show that "DeepN-JPEG" can achieve ~3.5x higher compression rate over the popular JPEG solution while maintaining the same accuracy level for image recognition, demonstrating its great potential of storage and power efficiency in DNN-based smart IoT system design.

==> analysis.tex <==
\section{Theoretical Analysis}
%In this section we explore which part of the image is redundant for training DNN model. 
% Then we analysis the two types of errors occurs at image compression: coefficients discard error and the roundoff error. Base on that we discussed the limitation of JPEG compression in DNN which is induced by discard error. At last we give some interesting observations of the roundoff errors happens on DNN based on our experimental results.   

% \subsection{Image at Frequency Domain in DNN}
% Modern compression technology design is based on human vision system.
% Those technologies are trade off image information with human vision effect. For example, one approach of JPEG compression technology achieve high compression rate is by assembling more high frequency component coefficient to zero. Then instead of write the coefficient values equal to zero we just write the number of zeros to compression files. Therefor the more coefficient equal to zeros the higher compression rate will achieve. The reason is human are more sensitive to the low frequency components of an image than high frequency ones. 

%  Generally speaking frequency of an image represent the intensity of changes on gray level, it can be understand as the gradient of the gray level at spacial domain. Different frequency components at an image have different effect. Low frequency components consist the gray level of an image, medium frequency components determine its structure, then hight frequency ones represent its edge and details which can be consider as the complement of medium ones. Then we try to explore whether DNN has less sensitivity for high frequency components as human vision. 
 
% We first try the human suitable compression method JPEG to verify the feasibility of this method used in DNN training process. As introduce in section~\ref{pre} we select three different quantization factor to scale the training dataset, i.e. (QF = 20, 50, 80), and  explore the effect. We choose the ImageNet ILSVRC2012  dataset and AlexNet network as our framework. The training dataset without compression process we call it original image. We use Independent JPEG Group to compress the training dataset. 
% The testing results shown in Fig.~\ref{jpegacc} indicates after 53 epochs training no matter how much the training images are compressed the testing top-1 accuracy still can't achieve the original images trained model.

% \begin{figure}[b]
% \begin{centering}
% \includegraphics[width=1\columnwidth]{figures/jpegacc}
% \end{centering}
% \caption{Top-1 accuracy of JPEG compression at different QF.}
% \label{jpegacc}
% \end{figure}
% It is understandable since JPEG is a lossy compression technology. The information loss happened at quantization step on the frequency components(FC).  We try to explore whether the  We first dig the weights after different training 
% % Natural image formed by intricate pattern, complicated objective edges and different color or luminance. Various images present large amount of information. DNN treat images as numbers of each pixel value. However it's really hard to find some rules or characteristics at spatial domain based on the pixel values. For example. same objective may have different shape, size, position and etc, while different objectives have more differences. 

% It's well known the human is more sensitive for the low frequency components of an image and can not discover the changes from high frequency part. Does the DNN has the same response as human? Consider we have a 8*8 gray image for simplify, Fig.~\ref{dct} describe the representation of one pixel value of this image at frequency domain: 
% \begin{equation}
% \label{eq_pix}
% p_{(i,j)}=\sum_{m=0} ^{m=7}\sum_ {n=0} ^{n=7} c_{(m,n)}\cdot b_{(m,n,i,j)}
% \end{equation}

% where $p_{(i,j)}$ is one pixel value of the 8*8 image, $c_{(m,n)}$ is the corresponding 8*8 coefficients after DCT, $b_{(m,n,i,j)}$ is the basis function at different frequency. Right 64 sub-blocks are the basis functions used for 8*8 DCT, we can see horizontal frequencies increase from left to right, and vertical frequencies increase from top to bottom. And each basis function is linearly independent that means the basis is unique can not be compound by others. The top-left white block has the same value is DC components as mentioned in previous section and the others are AC components have similar absolute values. 

% So each pixel is the linear accumulation results of corresponding position at basis function at every frequency. We discuss two descend dimension method convolution and max pooling which are widely used in DNN. Then the output of convolutional layer is the accumulation of each pixel value multiply the convolution kernel: 
% \begin{equation}
% \label{eq_con}
% o=\sum_{i=0} ^{i=3}\sum_ {j=0} ^{j=3} p_{(i,j)}\cdot k_{(i,j)}
% \end{equation}
% where $o$ is the output after convolution operation, $k_{(i,j)}$ is the convolution kernel. Since each pixel has the every frequency basis component, the output of the convolution layer does not flit the hight frequency components at forward process. After training some kernels may amplify the low frequency components, others may amplify the high frequency ones. At max pooling process, the largest value in the pre-defined regain is picked as the output. No matter which value is picked, the value composited by all the frequency components. Other layer like ReLu, fully connected, softmax, etc. does not discard any values. So the DNN is different compare to human visual system, combine Eq.~\ref{eq_pix} and Eq.~\ref{eq_con} we conclude DNN make response to every frequency components. 

% \begin{figure}[t]
% \begin{centering}
% \includegraphics[width=1\columnwidth]{figures/dctvision}
% \end{centering}
% \caption{One pixel at frequency domain representation.}
% \label{dct}
% \end{figure}


% However the coefficients at hight frequency components are usually small in natural image. That means the hight frequency components has small contribution to the over all image representation. Now we use experimental results prove how the high frequency components impact the neural network. Fig.~\ref{hfrm} shown the results of a well trained model with two images testing. The left one is the original image and the output of the model predict it as junco with a low confidence of $18.94\%$. Then we remove the high frequency components of this image and test it again, the output of the same model predict it as robin with $15.63\%$. However as human we can't see any difference from those two images.

% From our experimental results we can see, remove the high frequency of the image will reduce the confidence of the prediction. Therefore for some images with low prediction confidence this change may make wrong output. 

% \begin{figure}[t]
% \begin{centering}
% \includegraphics[width=1\columnwidth]{figures/highfrm}
% \end{centering}
% \caption{Image with and without high frequency comparison.}
% \label{hfrm}
% \end{figure}

% As all of the analysis above, we want conclude that all the 63 AC basis function or frequency components have same effect to neural network. Because: first DNN is processing numbers and all the AC frequency components no matter high or low are linear independent and have the similar absolute values, second on every step in DNN does not discard any frequency components, and last even the high frequency components usually have very small weights or coefficient values it still impact the DNN output. So DNN is not like human visual, it take response with ever frequency components. 

\subsection{The Difference between HVS and DNN}

\begin{figure}[t]
\begin{centering}
\includegraphics[width=1\columnwidth]{figures/quancompare}
\end{centering}
\caption{Original coefficient distribution and after de-quantization at different quantization value coefficient distribution.}
\label{q_compare}
\end{figure}

We have initialized our studies on an interesting problem: \textit{What are the major differences of image processing between human vision system and deep neural network?} This should help on explaining the aforementioned accuracy reduction issue, thus to guide the development of DNN-favorable compression framework. \textit{Our observation is that DNNs can response to any important frequency component precisely, but human visual system focuses more on the low frequency information than high frequency ones, indicating fewer features to be learned by DNNs after the compression.} 
 
Assume $x_k$ is a single pixel of a raw image \textbf{X}, and $x_k$ can be represented by $8\times8$ DCT in JPEG compression: 
\begin{equation}
x_k=\sum_{i=0} ^{i=7}\sum_ {j=0} ^{n=7} c_{(k,i,j)}\cdot b_{(i,j)}
\end{equation}
where $c_{(k,i,j)}$ and $b_{(i,j)}$ are the DCT coefficient and corresponding basis function at 64 different frequencies, respectively.
Because the human visual system is less sensitive to high frequency components, a higher CRatio can be achieved in JPEG compression by intentionally discarding those high frequency parts, i.e. zeroing out the associated $c_{(k,i,j)}$ through the scaled quantization. On the contrary, DNNs examine the importance of the frequency information in a quite different way. The gradient of the DNN function $F$ with respect to a basis function can be calculated as:
\begin{equation}
{ \frac{\partial F}{\partial b_{(i,j)}}=\frac{\partial F}{\partial x_k}\times\frac{\partial x_k}{\partial b_{i,j}}=\frac{\partial F}{\partial x_k}\times c_{(k,i,j)} }
\end{equation}
thus implying that the contribution of a frequency component ($b_{i,j}$) of a single pixel $x_k$ to the DNN learning will be mainly determined by its associated DCT coefficient ($c_{(k,i,j)}$) and the importance of the pixel ($\frac{\partial F}{\partial x_k}$). Here $\frac{\partial F}{\partial x_k}$ is obtained after the DNN training, while $c_{(k,i,j)}$ will be distorted by the image compression (i.e. quantization) before training. 
If $c_{(k,i,j)}=0$, the frequency feature ($b_{i,j}$), which may carry important details for DNN feature map extraction, cannot be learned by the DNN to update the parameters, thus limited accuracy:
\begin{equation}
\label{eq_act}
\triangledown w'_{i,j} =\frac{\partial (J(w\cdot \epsilon)-T)}{\partial w_{i,j}}
\end{equation}
where $\epsilon$ is the input error introduced by the feature degradation, J is the functionality of neural network and T is the target.

\begin{figure}[t]
\begin{centering}
\includegraphics[width=1\columnwidth]{figures/highfrm}
\end{centering}
\caption{Image with and without high frequency comparison.}
\label{hfrm}
\end{figure}

It is often the case in a highly compressed JPEG image, since $c_{(k,i,j)}$s of high frequency parts (usually small in nature images) are quantized to zero to ensure a better CRatio. 
Fig.~\ref{q_compare} shows the quantization induced feature degradation. With a moderate CRatio, i.e. QF = 80, the de-quantized coefficient distribution is similar to the original one but little sparse. However increasing the CRatio, i.e. QF = 60/20, is resulting in the over-sparse coefficients. 
As a result, DNNs can easily misclassify aggressively compressed images if their original versions contain important high frequency features. In CASE 1 (see Fig.~\ref{acc}(a)), the DNN model trained with original images learns comprehensive features, especially high frequency ones important for some images, however, such features are actually lost in some more compressed testing images, causing considerable misclassification rate. Fig.~\ref{hfrm} demonstrates such an example--the ``junco" is mis-predicted as ``robin" after removing a few high frequency components, despite that the differences are almost indistinguishable by human eyes. In CASE 2 (see Fig.~\ref{acc}(b)), the model is trained to make decisions solely based on the limited number of features learned from more compressed training images, and the additional features in high quality testing images cannot be detected by DNN for accuracy improvement. 



% In this section  

% We want the training image size as small as possible to achieve our goal. As introduce in section~\ref{pre} JPEG is the most widely used and proven technique for image compression. Five different quantization factor that is used to scale the quantization table to achieve different compress rate (QF = 10, 20, 50, 70, 90) is chosen to explore the effect of JPEG in DNN. We use ImageNet as input dataset, AlexNet as DNN architecture and the original validation dataset is used for all models testing. 
% The results shown in Fig.~\ref{jpegacc} indicate after 53 epochs training no matter how much the training images are compressed the testing top-1 accuracy still can't achieve the original images trained model. 
       



% JPEG failed for directly used in DNN for input dataset compression. In order to explore the reason the original dataset trained model we call it $\it{model\_ori}$ and using $QF = 10$ compressed dataset trained model called $\it{model\_comp}$ is picked for analysis. Also random selected one validation image and its compressed version are fed into the $\it {model\_ori}$ and $\it{model\_comp}$. We count the output of last convolutional layer feature maps after the different images fed to different DNN models. The results are shown in Table~\ref{feat_map}, we use number of features that the content are all zeros to determine how many features the model can detect. For example the compressed image feed to $\it {model\_ori}$, then the last convolutional layer has 49 content are all zeros feature maps. So less number means more feature can be detected. $\it {model\_comp}$ always have less feature maps can be detect compare to $\it {model\_ori}$ that is it can not recognition some feature like $\it {model\_ori}$ do. We assume that's because compression process loss some feature at input dataset. 


% \begin{table}[t]
% \centering
% \caption{Last convolutional layer feature map comparison.}
% \label{feat_map}
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{|c | c | c |} 
%  \hline
%  Number of zeros & img\_comp & img\_ori  \\ 
%  \hline\hline
%  Model\_comp & 63 & 64  \\ 
%  \hline
%  Model\_ori & 49 & 40  \\ 
%  \hline
% \end{tabular}%
% %}
% \end{table}

% The JPEG is lossy compression technology and the quantization step is where the information loss. From Eq.~\ref{eq_quan} after the coefficient divided by its quantization value (QV) the result are round to its nearest integer. When the image is decompressed to row data the rounded integer will multiply by the same quantization value. However de-quantized value is not the exactly value before since the decimals are discarded at divination operation that's how the error induced.   
% Fig.~\ref{q_compare} illustrate the quantization induced error. The left top figure is one coefficient distribution before quantization and the rest of the three is this coefficient distribution using different quantization value. At QV = 50 the de-quantized coefficient distribution is similar to the original but little sparse. As the QV increase the  distribution become more sparse. On the bottom right figure, the majority of the coefficients are become zeros that's there is no such frequency components feed to the neural network. It's obvious the larger the quantization value the more error will induce.
% \begin{figure}[b]
% \begin{centering}
% \includegraphics[width=1\columnwidth]{figures/quancompare}
% \end{centering}
% \caption{Original coefficient distribution and after de-quantization at different quantization value coefficient distribution.}
% \label{q_compare}
% \end{figure}

% By investigating the quantization table what is JPEG used we can see the quantization values in the table has the increase trend from top left to bottom right. This is because quantization table in JPEG is designed by human vision system. So to improve compress rate the coefficient are quantified to zero from higher frequency to lower one. As the QF become smaller the value in the quantization table become large and more coefficients will be quantized to zero. It can be considered as the compressed input dataset can only provide a part of input pattern or input feature. So some pattern at high frequency components will not be learned by neural network: 

% \begin{equation}
% \label{eq_act}
% \triangledown w'_{i,j} =\frac{\partial (J(w\cdot \epsilon)-T)}{\partial w_{i,j}}
% \end{equation}

% where $\epsilon$ is the error of input due to the high frequency components are removed, J stand for the functionality of the neural network and T is the target.

% Now we want prove the accuracy degradation is caused by the high frequency components loss at input dataset. For a well trained $\it model\_comp$ we test the accuracy of both original and compressed validation dataset. Since limited input features are provide to the neural network the $\it model\_comp$ will response for limited pattern from input dataset. Therefore even original validation dataset are used for testing $\it model\_comp$ will have no response for the extra input feature it does not learned. It means the compressed dataset and the original dataset will have the same testing accuracy for a $\it model\_comp$. Table~\ref{comp_ori_acc} shown the experiential results, $\it model\_comp10$ meaning the neural network model is trained by QF = 10 images dataset and so on, $\it img\_comp$ stand for the testing images have the same QF as the training image, and $\it img\_ori$ is the original testing images. The results shown the compressed and original testing images always have the same testing accuracy. It's proved our understanding that high frequency components loss in input dataset lead to the DNN can't learned the corresponding pattern. 

% Overall of this section, we first find the JPEG compressed dataset can't ensure the training model accuracy. Further investigation shown compressed model will loss features caused by JPEG compression discard high frequency components for compress. Then we proved DNN can learn the detailed information of image high frequency components. 


\begin{table}[b]
\centering
\caption{Different model testing on corresponding compressed image and original image.}
\label{comp_ori_acc}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{|c | c | c |} 
 \hline
 Accuracy(\%) & img\_comp & img\_ori  \\ 
 \hline\hline
 Model\_comp10 & 48.99 & 48.97  \\ 
 \hline
 Model\_comp20 & 51.46 & 51.56  \\ 
 \hline
  Model\_comp50 & 53.28 & 53.35  \\ 
 \hline
  Model\_comp70 & 53.73 & 53.6  \\ 
 \hline
  Model\_comp90 & update & update  \\ 
 \hline
\end{tabular}%
%}
\end{table}

% \subsection{Error Tolerance for Feature Degradation}
% From previous analysis every frequency components can be learned form DNN. In order to ensure the accuracy we can't discard any frequency components. 

% From our analysis previously after input images go through quantization and de-quantization steps some high scaled coefficients may loss high frequency components and even other light scaled coefficients also induce errors. Since DC component indicate the luminance of a sub-block and AC components represent the pattern, here we only analysis the AC components. We proved loss frequency component can lead to accuracy reduction. We will analysis if this error induced light scaled coefficients cause the accuracy degradation. The error generated from the light scaled coefficients can be deduced as:
% \begin{equation}
% \label{eq_act}
% C_1 = DCT(I)  = DCT([IDCT(C'_1)])= DCT(IDCT(C'_1)+r) =  C'_1+\epsilon
% \end{equation}
% where $[]$ means round operation, I is the raw image, $C_1$ is decompressed coefficient from input JPEG image, $C'_1$ is de-quantized coefficient, $r$ is error from round operation and $\epsilon$ is the induced error. From \cite{JPEG Quantization Step Estimation and
% Its Applications to Digital Image Forensics}  the round-off error $\epsilon$ is assumed to be Gaussian distributed with zero-mean and variance $\frac{1}{12}$: 


% \begin{equation}
% \label{eerr}
% \epsilon\sim \it N(0,\frac{1}{12})
% \end{equation}

% Suppose two image dataset under specific compress rate to ensure both of the datasets have same frequency components.
% For one of them we add error form Eq.~\ref{eerr} and another don't change to training two set of models, for the sake of understand how this AC error can impact DNN. 

% Fig.~\ref{fre} shown the experimental result. From this experiment we chose both of the input data set under QF = 10 compress condition. For one of the dataset we add error as mentioned before. After each epoch finished we use the same validation images to test the accuracy of the corresponding model. The results clearly shown light scaled coefficients induced errors has no effect on the DNN model. 

% Therefore we conclude our observation as: first, DNN take response for every frequency components. So in order to ensure the model  accuracy any frequency components can not be discarded. Second, DNN can tolerance some degree of errors. It's indicate every frequency components should be keep, however those components can have some error without accuracy loss
% . 




% \begin{figure}[b]
% \begin{centering}
% \includegraphics[width=1\columnwidth]{figures/fre}
% \end{centering}
% \caption{QF = 10  with and without error dataset trained model.}
% \label{fre}
% \end{figure}

% We will analysis if this error induced light scaled coefficients cause the accuracy degradation and how much error each band can tolerance. To evaluate each frequency components is costly, thus inspired from ~\cite{kaur2011steganographic} which indicate the frequency components can be broken up into three bands, i.e., LF--low frequency band, MF--middle frequency band and HF-- high frequency band as shown in left part of Fig.~\ref{fre}. 

% We directly change the values used in un-/quantization steps for each band with an interval as 5 and keep the rest QV in other bands with value 1. The results is shown in the right part of Fig.~\ref{fre}, apparently large quantization value will induce more error since it may round off larger values. From the figure we can see the LF band is more error sensitive after QV is larger than 10. This is reasonable since coefficients in LF are large which is more important to DNN. While larger QV at MF/HF will impact the accuracy and the accuracy will maintain when the QV is larger. This is because several classes at training dataset have relative large frequency coefficients thus large QV will decrease the accuracy for those classes.  

% Therefore we conclude our observation as: first, DNN take response for every frequency components. The larger coefficients will impact the DNN accuracy more. Second, DNN can tolerance some degree of errors dependents on the value of coefficients. It's indicate every frequency components should be keep, however those components can have some error without accuracy loss. 





















